Lost in Interpretation: Navigating Challenges in Validating Persistency Models Amid Vague Specs and Stubborn Machines, All with a Sense of Humour

Memory persistency models provide a foundation for persistent programming by specifying which (and when) writes to non-volatile memory (NVM) become persistent. Memory persistency models for the Intel-x86 and Arm architectures have been formalised, but not empirically validated against real machines. Traditional validation methods %such as %extensive litmus testing used for memory \emph{consistency} models do not straightforwardly apply because a test program cannot directly observe when its data has become persistent: it cannot distinguish between reading data from a volatile cache and from NVM. We investigate addressing this challenge using a commercial off-the-shelf device that intercepts data on the memory bus and logs all writes in the order they reach the memory. Using this technique we conducted a litmus-testing campaign aimed at empirically validating the persistency guarantees of Intel-x86 and Arm machines. We observed writes propagating to memory out of order, and took steps to build confidence that these observations were not merely artefacts of our testing setup. However, despite gaining high confidence in the trustworthiness of our observation method, our conclusions remain largely negative. We found that the Intel-x86 architecture is not amenable to our approach, and on consulting Intel engineers discovered that there are currently no reliable methods of validating their persistency guarantees. For Arm, we found that even a machine recommended to us by a persistency expert at Arm did not match the formal Arm persistency model, due to a loophole in the specification.

==> 3.infrastructure.orig.tex <==
\section{Empirical Infrastructure}

To explore the recoverability behaviour in normal operation, it is necessary to monitor the order in which data updates are made persistent, meaning when they reach the non-volatile memory (NVM). Achieving this goal requires real-time visualisation of the persistence domain. In the context of ARM architecture, the persistence domain is synonymous with persistent memory, denoting the absence of any other battery-backed memory/cache unit. Nonetheless, accurately accessing memory signals to visualise the state of the DDR command bus can be a challenging task.

One of the endorsed practices to gain insight into DDR bus activity and establish direct access to memory signals is through the use of chip interposers. These interposers provide probing and monitoring capabilities, allowing for the observation of signals on the DDR bus.
The FS2800 \DDRDetective{} from FuturePlus Systems \cite{FuturePlus} is an example of a memory bus interposer that enables direct access to memory signals and offers insights into DDR bus activity. It allows for close-proximity probing of persistent memory and acts as a repeater, providing non-intrusive protocol decode of memory transactions and state analysis. Its logic analyser serves as the analysis execution engine, commonly known as the \emph{probe manager}. The setup process for the interposer probe is simple, with it snapping onto the motherboard, and the memory component then attaching to the top (depicted schematically in \cref{fig:setup}). 
Through this approach, it becomes possible to monitor traffic and process JEDEC\footnote{JEDEC (Joint Electron Device Engineering Council) is the engineering standardisation body that develops open standards and publications for the microelectronics industry, including DDR4.} DDR4 memory protocol requirements in real-time.
The bus analysis probe offers triggers for detecting state violations and user-selectable DDR commands or command sequences to enhance system analysis.
%This allows to explore recoverability behaviour with respect to durability and ordering in normal operation.



\subsection{Overall Flow}

The present study proposes a methodology, the schematic overview of which is depicted in \cref{fig:flow}. This process involves a cross-program invocation mechanism, whereby the conductor program, AutiIt\footnote{\url{www.autoitscript.com}} (see \cref{subsec:impl_challenges}), calls instructions from other programs in a predetermined temporal sequence. The main constituents of this methodology encompass the following steps.



\begin{figure*}
\captionsetup{width=1\textwidth}
\includegraphics[width=1\textwidth]{experimentSetup}
  \caption{The flow of validating the persistency semantics; a colour nested inside another denotes an embedded program within outer code; a hexagon allows the flow to continue if the condition inside is true}
  \label{fig:flow}
\end{figure*}


\begin{litmustest}   

\caption[Caption for LOF]{A litmus test in ARMv8.2 preceded by the corresponding preamble; the \texttt{asm} keyword declares inline assembler instructions that are embedded within the \texttt{C} code; $x_{pd}$ denotes the value of $x$ read from the persistence domain utilising physical probing}\label{alg:mthread}

\hspace*{-.25cm} \includegraphics[width=\columnwidth]{litmus_test}
\vspace*{.01cm}
 
\end{litmustest}




\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle, fill=black, text=white, draw,inner sep=2pt] (char) {#1};}}

%\begin{list}{$\arabic$}{\leftmargin=1em \itemindent=0em}
\begin{list}{\protect\circled{\arabic{qcounter}}}{\usecounter{qcounter} \leftmargin=2.2em \itemindent=0em}
  \item The initial step of the proposed methodology involves the creation of persistency litmus tests, utilising the Alloy-encoded declarative models specific to either the Intel architecture \cite{RaadWNV20} or ARM architecture \cite{RaadWV19}. These tests represent instances that the underlying SAT engine of Alloy found to be satisfactory. 

    To provide further support for our validation process description, we utilise \cref{alg:mthread}, a specialised variant of \cref{alg:Arm} designed for automation.

\begin{comment}
    \begin{myquote}{Litmus Test 1}
    The program contains a synchronisation mechanism using the $\mathit{dsb(sy)}$ (full system Data Synchronisation Barrier) instruction in the left thread, which ensures that the write operation on $x$ is completed and persisted before the write operation on $y$. Specifically, the $\mathit{dsb(sy)}$ instruction acts as a memory barrier that prevents the reordering of instructions and waits for the completion of the $\mathit{dc\_cvap(x)}$ operation before allowing the write operation on $y$ to proceed. Therefore, if $y$ is equal to $\mathit{reg}$ upon recovery (i.e., the write operation on $y$ has persisted before the crash), we can infer that $x$ is also equal to $\mathit{reg}$ (i.e., $\mathit{dc\_cvap(x)}$ and the write operation on $x$ have also completed and persisted before the crash).
    
    In the right thread, when $y$ is read as $\mathit{reg}$ (which was written by the left thread), the ARMv8.2 model ensures that $y \leftarrow \mathit{reg}$ is ordered before $a \leftarrow y$. Thus, since $x \leftarrow \mathit{reg}; \mathit{dc\_cvap(x)}; \mathit{dsb(sy)}$ is executed before $y \leftarrow reg$, we can infer that $y \leftarrow \mathit{reg}$ is ordered before $a \leftarrow y$, and $z \leftarrow \mathit{reg}$ is ordered after $a \leftarrow y$ (due to the intervening $\mathit{dsb(sy)}$ instruction). Therefore, we can conclude that $x \leftarrow \mathit{reg}; \mathit{dc\_cvap(x)}; \mathit{dsb(sy)}$ is ordered before $z \leftarrow reg$. Consequently, if $z$ is equal to $\mathit{reg}$ upon recovery (i.e., $z \leftarrow \mathit{reg}$ has persisted before the crash), we can infer that $x$ is also equal to $\mathit{reg}$ (i.e., $x \leftarrow \mathit{reg}; \mathit{dc\_cvap(x)}$ must have also persisted before the crash).
    
    However, it's important to note that if a crash occurs after $z \leftarrow \mathit{reg}$ has executed and persisted but before $y \leftarrow \mathit{reg}$ has persisted, it's possible to observe $y=0$ and $z = \mathit{reg}$ after recovery, even though $y=0$ and $z=\mathit{reg}$ are never possible during normal (non-crashing) executions. This is because $y\leftarrow \mathit{reg}$ may persist after $z\leftarrow \mathit{reg}$. Therefore, we need to be careful when interpreting the observed values of $y$ and $z$ upon recovery.
    
    \end{myquote}
\end{comment}

  The litmus test is complemented by a post-recovery property, which confines the admissible outcome of the test. 
  In \cref{alg:mthread} this property is articulated as an assertion on the plausible values of (shared) memory locations $x$ and $y$ following recovery.
  %outcome, expressed as a constraint on the program’s final state.
  \item Subsequently, we issue instructions to the \DDRDetective{} to initiate the trigger solely on the WR (write) Commands. This entails that upon detection of the trigger condition (i.e., the initial write instruction to be issued by the litmus test), the probe will capture all subsequent commands up to a predetermined depth in the trace memory.
  \item Upon initiation of data capture, the Probe Manager host initiates a remote \texttt{ssh} tunneling with the target system to invoke the litmus test script.
  In the preamble of said script, a block of memory, which is ensured to be aligned to the size of the CPU cache line, is acquired for every memory location referenced in the litmus test. The starting (base) address of each block of memory is then stored in pointers to volatile variables that are used in the specific litmus test being executed (see \cref{alg:mthread} lines 1, 2).\\
We opted to allocate memory blocks that are aligned to the size of CPU cachelines to address a potential interference issue we observed during litmus testing. 
Specifically, we noticed that the number of writes propagated to the memory, as recorded in the \DDRDetective{} log, was unexpectedly higher than the number of writes issued by the litmus test at that location (see \cref{sec:evaluation}). 
This suggested the presence of other instructions that could potentially interfere with the litmus test.
In the hope to prevent such interference, we aligned the memory allocation to the cacheline size and allocated contiguous chunks of memory, each consisting of a multiple of cachelines. 
By doing so, we could ensure that no instruction other than the one committed by the litmus test would reside in any cacheline of the allocated chunks.
This allocation strategy guarantees that any issues observed during the litmus test are solely attributable to the committed instruction, thus improving the accuracy and reliability of the results.
As discussed in \cref{sec:evaluation}, the phenomenon of the number of propagated instructions exceeding the number of issued instructions was found to be specific to ARMv8.2 architecture; we did not observe this behavior in x86 architecture.\\
To enhance the experiment's interest, we deliberately designated the sizes of the allocated arrays to ensure that they spanned both L1 and L2 caches. 
The preamble then issues multiple writes to the designated memory locations using a predetermined frequency ratio, such as the $x:y$ ratio of $1:2$ used in \cref{alg:mthread}.
Upon the completion of the preamble, the script execution is intentionally paused  for a specified duration to allow steps \circled{4} to \circled{6} to complete.
\item After activating the probe (as described in step \circled{2}) and initiating the litmus test preamble (as described in step \circled{3}), the \DDRDetective{} records and logs instances of write-commands in a \singleq{geometric} pattern.\footnote{Memory arrays are organised into rows and columns of memory cells, which are referred to as \emph{wordlines} and \emph{bitlines}, respectively. The intersection of a wordline and a bitline uniquely identifies each memory cell's location within the array.} 
Upon satisfaction of the trigger condition, the captured data is exported as a CSV file, and the resulting log file will include all DRAM geometric locations that correspond to the writes issued during the preamble.
\item Afterwards, a Python script will scan the stored data file to identify DRAM locations that match the frequency ratio set in the preamble (as described in step \circled{3}).
To achieve this, the script initially groups all writes by their corresponding memory location into equivalence classes, then sorts the total number of writes for each location in ascending order. Using a ratio approximation of 1:2, the script deduces which DRAM location represents which memory location allocated in the litmus test. 
Notably, the script's logic remains invariant to the frequency and duration of the writes specified in the litmus test's preamble.
This process enables us to establish the mapping from the OS addresses allocated in the litmus test to their corresponding DRAM geometric locations.
\item After translating the system addresses into DRAM locations, we compute a bit-sequence (see \S  \ref{subsec:impl_challenges}) that preserves the bits that match between the binary representations of the geometric DRAM locations identified in the previous step, while treating non-matching bits as don't-care-bits. This generates a bit mask that covers all the memory locations that appear in the litmus test.
We then initiate a fresh capture of write-commands by explicitly directing the probe to record only at the locations that correspond to the computed wildcard bitmask.
\item Afterwards, the litmus test script will be activated and execute the post-preamble part, which constitutes the actual litmus test, repeatedly for a predetermined duration of time.
\item The probe will continuously capture data based on the storage criteria set in step \circled{6} until the trace buffer reaches its predetermined record size.
%until the memory is full.
\item As we utilise a wildcard bitmask to match the DDR locations corresponding to the memory allocated in the litmus test, only a subset of the log (exported in the previous step) matches this criterion. To remove the noise from the trace, a Python script will filter the log by the geometric addresses reverse-engineered in step \circled{5}.

  %If a signal meets the requirements expressed in the filter, then it is displayed in the list of signal. 

  
\item Ensuring the satisfaction of the post-recovery property in the litmus test (line 19 in \cref{alg:mthread}) can be reduced to the task of scrutinising the order in which the test's writes to memory locations are persisted. In \cref{alg:mthread}, the post-recovery property is equivalent to the assertion that, in every iteration of the litmus test, it is impossible for $y$ to be persisted before $x$, effectively fulfilling the requisite ordering condition.\\
It's worth noting that programmatically checking the post-recovery property is not possible because a running program cannot directly observe when its data has become persistent. This makes it difficult for the program to determine whether it is reading values from a volatile cache or from persistent memory. As a result, the responsibility of verifying the post-recovery property falls on the post-processing of the tracer obtained from the \DDRDetective{}.

\end{list}

% allocate a chunk of physically contiguous virtual memory which resides in lowmem (a zone in kernel space).




\subsection{Key Challenges}

Validating persistency semantics on real machines is a daunting task, primarily due to the intermediation of caches between the program and the persistence domain, which adds to the complexity.
Furthermore, throughout our research journey, we encountered several other obstacles that required us to address them in an ad hoc manner, devise clear solutions and adjust our approach accordingly. Below, we outline few of these challenges and the proposed solutions.

\noindent\textbf{Mapping Virtual Addresses to DRAM Addresses }
The \DDRDetective{} employs an analysis of DDR4 bus traffic by referencing the underlying \singleq{geometric} locations of DRAM.
A DRAM address is a 7-tuple that comprises {\tt <\,channel}, {\tt DIMM}, {\tt rank}, {\tt bank group}, {\tt bank address}, {\tt row}, {\tt column\,>}, arranged in a specific order that reflects the memory chip's hierarchy levels and geometry. 
In our experiments, we use only one DIMM plugged in at a time which means that the last four elements of the tuple (bank group, bank address, row, and column) are sufficient to identify a DRAM address uniquely.\footnote{Memory arrays are organised into rows and columns of memory cells, which are referred to as \emph{wordlines} and \emph{bitlines}, respectively. The intersection of a wordline and a bitline uniquely identifies each memory cell's location within the array.} 

For the allocated OS virtual memory to be useful, it must be mapped to its corresponding DRAM location. However, the specifics of this mapping are often considered proprietary information and kept as trade secrets, resulting in a lack of documentation and information. 
As a consequence, mapping system virtual addresses to specific rows, columns, and banks in DRAM can be a challenging task, since the necessary details for the mapping process are not readily available.

Conceptually, one approach to deducing the mapping between an OS address and its corresponding physical location in DRAM would involve triggering the \DDRDetective{} tool on the \emph{value} assigned to a specific address, then examining the trace buffer for the corresponding entry. However, in practice, this approach is not feasible due to a limitation of the \DDRDetective{} tool. 
Specifically, the \DDRDetective{} cannot trigger on a value assigned to a specific address in memory because it lacks access to the \emph{data signals}. Therefore, this method is not suitable for deducing the mapping between system virtual addresses and their locations in DRAM.

Prior research \cite{9152654, 10.1145/3466752.3480069, 10.1109/ISCA45697.2020.00059, DRAMA, 10.1145/3084464, 10.1145/2989081.2989114,10.1007/978-3-030-00470-5_3} aimed to reverse engineer this map mainly using RowHammer attacks\footnote{RowHammer attacks exploit the fact that accessing a specific memory row (the aggressor row) induces the highest number of bit flips in the adjacent memory rows. This knowledge can then be used to potentially compromise the system. As a result, the mapping scheme is often kept undocumented by vendors to prevent attackers from exploiting it.}, but also employed other approaches such as side-channel attacks, reduced timing parameters, thermal heaters, physical probing, or a combination of these techniques.
%
%mapping is confidential -- The address mapping isn't documented --  address mapping may vary among different mother boards even they have the same generation of CPU 
%

In contrast to previous methods, we took a different approach and leveraged \DDRDetective{} hardware to employ a more straightforward end-to-end approach for reverse engineering the mapping scheme.
With the \DDRDetective{} running, we issue multiple writes to each memory location that appears in the litmus test on a ratio of $1:2:3\dots$
We then inspect the \DDRDetective{} log to identify geometric DRAM locations in the same ratio. For example, in the preamble of \cref{alg:mthread}, writes to memory locations $x, y, z$ are committed on a ratio of $1:2:3$, respectively.
It's important to note that our method provides only a partial mapping, which maps only the memory locations present in the litmus test.
To obtain a complete mapping, one can populate a lookup table where the inputs are the OS memory addresses and the outputs are the physical DRAM addresses logged in the \DDRDetective{} for the given input. The lookup table can then be converted to Algebraic Normal Form (ANF) by performing a brute-force search of linear functions to derive the mapping function. Similar approach is presented here \cite{DRAMA}.
However, it's worth noting that for our work, a complete mapping was not necessary.

\subsection{Implementation Challenges}\label{subsec:impl_challenges}

\noindent\textbf{Automation } The probe manager application of the \DDRDetective{} lacks command-line interface (CLI) support and relies solely on a Windows graphical user interface (GUI). This limitation poses a significant challenge for automation of experiments and remote access. To surmount this challenge, we resorted to leveraging AutoIt, a scripting language designed to facilitate automation of the Windows GUI and general scripting tasks. AutoIt achieves this by simulating keystrokes, mouse movements as well as window and control manipulations, enabling effective automation of tasks that require interaction with the Windows GUI.


\noindent\textbf{Storage Qualification Limitation } One additional challenge we encountered with the probe manager application was its inability to accept more than one DRAM location tuple as storage qualification.\footnote{In FuturePlus Systems\cite{FuturePlus} terminology, the field in the \emph{Probe Manager} application of the \DDRDetective{} where the criteria for logging intercepted memory instructions is entered is referred to as Storage Qualification.} 
This means that the application could only capture and log one specific address at a time, corresponding to a single variable that we wrote during the litmus test. 
%As a reminder, each geometric DRAM location tuple corresponds to one variable for which we commit writes in the litmus test. 
To address this limitation and enable the logging of additional variables, we devised a solution by computing a bitmask that treats the non-matching bits between the binary representations of the geometric locations where shared memory locations are stored as 'don't-care-bits'. This enabled us to accommodate multiple variables using a single storage qualification field, effectively expanding the application's capabilities..
